Leveraging RGB-D Data with Cross-Modal Context Mining for Glass Surface Detection

Glass surfaces are becoming increasingly ubiquitous as modern buildings tend to use a lot of glass panels. This, however, poses substantial challenges to the operations of autonomous systems such as robots, self-driving cars, and drones, as these glass panels can become transparent obstacles to navigation. Existing works attempt to exploit various cues, including glass boundary context or reflections, as priors. However, they are all based on input RGB images. We observe that the transmission of 3D depth sensor light through glass surfaces often produces blank regions in the depth maps, which can offer additional insights to complement the RGB image features for glass surface detection. In this work, we first propose a large-scale RGB-D glass surface detection dataset, \textit{RGB-D GSD}, for rigorous experiments and future research. It contains 3,009 images, paired with precise annotations, offering a wide range of real-world RGB-D glass surface categories. We then propose a novel glass surface detection framework combining RGB and depth information, with two novel modules: a cross-modal context mining (CCM) module to adaptively learn individual and mutual context features from RGB and depth information, and a depth-missing aware attention (DAA) module to explicitly exploit spatial locations where missing depths occur to help detect the presence of glass surfaces. Experimental results show that our proposed model outperforms state-of-the-art methods.

==> macros.tex <==
\usepackage[dvipsnames]{xcolor}
\usepackage{makecell}
% \usepackage[normalem]{ulem}
\usepackage[normalem]{ulem}
\usepackage{multirow}
\definecolor{mygreen}{RGB}{0,180,0}
\definecolor{myyellow}{RGB}{153, 122, 0}
\newcommand{\jy}[1]{\textcolor{mygreen}{#1}}
\newcommand{\jychecked}[1]{#1}

\newcommand{\jiaying}[1]{\textcolor{myyellow}{\textbf{Jiaying:} #1}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
% \newcommand\redout{\bgroup\markoverwith
% {\textcolor{red}{\rule[0.5ex]{2pt}{0.8pt}}}\ULon}

\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\etal}{\textit{et al}.}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}
